TRCF: Temporal-Reference Complementary Forecasting for Irregular Multivariate Time Series

Irregular multivariate time series forecasting supports healthcare monitoring, environmental analysis, and activity recognition. Channel-independent (CI) approaches capture each variable's temporal patterns but do not explicitly use observations from other variables. Channel-dependent (CD) modeling exploits relationships among variables, yet asynchronous measurements make these relationships difficult to learn. Incorporating cross-variable information while preserving each variable's irregular history therefore remains a key challenge. We propose Temporal-Reference Complementary Forecasting (TRCF), a framework that augments a compact CI forecaster with a complementary CD branch. ANCHOR aggregates observed values and timestamps at shared temporal locations, retaining observation support to form compact CI features. BRIDGE constructs complementary features through history completion. It first estimates each variable's historical values from its own observations, then uses differences between other variables' observed and estimated values at nearby times to correct missing entries. The completed history preserves observed values and is encoded to supply context alongside the direct CI representation. Finally, the two representations are fused, combined with the query-time embedding, and passed to a shallow multilayer perceptron for forecasting. Experiments on four real-world datasets show that TRCF achieves the lowest mean squared error and mean absolute error in the main benchmark comparison, while reducing measured peak inference memory by 17.28% to 87.98% relative to APN.

==> sections/ai_disclosure.tex <==
% Disclosure removed at the author's request.


==> sections/new_module_results.tex <==
Removing ANCHOR raises MSE/MAE by 21.87\%/21.77\% on HA,
3.50\%/3.70\% on P12, and 2.44\%/2.50\% on MIMIC, with both
errors higher in every paired seed. These results establish the value
of the direct path within the complete predictor. They do not compare
alternative temporal encoders; Section~\ref{sec:encoder-comparison}
evaluates those separately.
Removing BRIDGE raises MIMIC MSE/MAE by 4.44\%/2.71\%; its effects
on HA and P12 are smaller. On USHCN, ANCHOR alone improves both
metrics, while BRIDGE alone has lower MSE but higher MAE than the
complete model. The combined paths improve both errors over either
path removal on three datasets under the stated recipe.


==> tables/completion_alternative.tex <==
\begin{table}[t]
\centering
\caption{Residual relay and raw sources filled with temporal estimates. Five-seed test means.}
\label{tab:completion-alternative}
\begingroup\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.18}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrrr@{}}
\toprule
Model & \multicolumn{2}{c}{HA} & \multicolumn{2}{c}{USHCN} & \multicolumn{2}{c}{P12} & \multicolumn{2}{c}{MIMIC} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
 & MSE $\downarrow$ & MAE $\downarrow$ & MSE $\downarrow$ & MAE $\downarrow$ & MSE $\downarrow$ & MAE $\downarrow$ & MSE $\downarrow$ & MAE $\downarrow$ \\
\midrule
\textbf{TRCF} & \numstat{0.04070}{0.000191143} & \numstat{0.11235}{0.000247643} & \numstat{0.14305}{0.010575315} & \numstat{0.25237}{0.005621037} & \numstat{0.28721}{0.000267297} & \numstat{0.35160}{0.000564862} & \numstat{0.40428}{0.003305092} & \numstat{0.38160}{0.000830660} \\
\midrule
Model-filled raw values & \numstat{0.04073}{0.000154694} & \numstat{0.11270}{0.000145665} & \numstat{0.14272}{0.010124163} & \numstat{0.25235}{0.005457580} & \numstat{0.28627}{0.000536853} & \numstat{0.35257}{0.000917840} & \numstat{0.40846}{0.002514023} & \numstat{0.38648}{0.002502749} \\
\bottomrule
\end{tabular*}
\endgroup
\end{table}


==> tables/context_parameters.tex <==
\begin{table}[t]
\centering
\caption{Trainable parameter counts; the historical reconstruction weight does not change the architecture.}
\label{tab:context-parameters}
\begingroup\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{2pt}\renewcommand{\arraystretch}{1.18}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Model & HA & USHCN & P12 & MIMIC \\
\midrule
ANCHOR & 21649 & 987 & 5265 & 4113 \\
Widened ANCHOR & 36339 & 6850 & 12174 & 19359 \\
Interpolated context & 36346 & 6843 & 12186 & 19375 \\
Temporal context & 36318 & 6873 & 12175 & 19358 \\
TRCF & 36292 & 6843 & 12164 & 19332 \\
\bottomrule
\end{tabular*}
\endgroup
\end{table}


==> tables/controlled_conditions.tex <==
\begin{table}[t]
\centering
\caption{Controlled signal and sampling regimes. Three-seed test MSE/MAE means.}
\label{tab:controlled-conditions}
\begingroup\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.18}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Condition & \multicolumn{2}{c}{ANCHOR} & \multicolumn{2}{c}{TRCF} & \multicolumn{2}{c}{Raw relay} & \multicolumn{2}{c}{Observed residuals} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
 & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
\midrule
indep., fast, async & \resultcell{0.4178}{0.0027064863987856774} & \resultcell{0.5139}{0.0020329975718468068} & \resultcell{0.3972}{0.0026097253880675393} & \resultcell{0.5001}{0.0011014453106323275} & \resultcell{0.3973}{0.0020442359253123265} & \resultcell{0.5000}{0.00098336127032414445} & \resultcell{0.3973}{0.0021935681241819589} & \resultcell{0.5002}{0.00081180875039003062} \\
indep., fast, sync & \resultcell{0.4265}{0.0029486684388469252} & \resultcell{0.5208}{0.0017417307079820119} & \resultcell{0.4099}{0.00079934350348815351} & \resultcell{0.5118}{0.00046967468082709983} & \resultcell{0.4097}{0.0016836994873667601} & \resultcell{0.5114}{0.00094213935308939457} & \resultcell{0.4100}{0.0011634785617689661} & \resultcell{0.5119}{0.00069290810062092912} \\
indep., persistent, async & \resultcell{0.3170}{0.015288392801778536} & \resultcell{0.4408}{0.010246039437147554} & \resultcell{0.2945}{0.0097795143178116949} & \resultcell{0.4245}{0.0056923152478942024} & \resultcell{0.3018}{0.010418389687744061} & \resultcell{0.4299}{0.00656617812281572} & \resultcell{0.2947}{0.0093826800917857448} & \resultcell{0.4247}{0.0053050474513197327} \\
indep., persistent, sync & \resultcell{0.3082}{0.011202256197069006} & \resultcell{0.4408}{0.0086841699752113529} & \resultcell{0.2935}{0.0073780411902709874} & \resultcell{0.4285}{0.0062915540844429357} & \resultcell{0.2926}{0.006056778837168591} & \resultcell{0.4282}{0.0052701699094670389} & \resultcell{0.2936}{0.0072746250611691581} & \resultcell{0.4285}{0.0062005329394856498} \\
shared, fast, async & \resultcell{0.4326}{0.0027008405480342169} & \resultcell{0.5211}{0.0015303104524785106} & \resultcell{0.4137}{0.0010459713006383483} & \resultcell{0.5100}{0.00041143899615862458} & \resultcell{0.4159}{0.0010769865606531932} & \resultcell{0.5115}{0.00035616930719526774} & \resultcell{0.4133}{0.0010279412450944381} & \resultcell{0.5099}{0.00029341091014576634} \\
shared, fast, sync & \resultcell{0.4349}{0.0031767869131874584} & \resultcell{0.5250}{0.0020778283714393353} & \resultcell{0.4178}{0.00061722374494548613} & \resultcell{0.5149}{0.00070181993988443667} & \resultcell{0.4174}{0.00052927943873035338} & \resultcell{0.5148}{0.00028826793763083255} & \resultcell{0.4174}{0.00066484428720845206} & \resultcell{0.5147}{0.00074116031284430898} \\
shared, persistent, async & \resultcell{0.3178}{0.011165670566009729} & \resultcell{0.4431}{0.0075874251841844386} & \resultcell{0.2957}{0.0051638142824892725} & \resultcell{0.4279}{0.0024712764935025697} & \resultcell{0.3034}{0.0062391732597753304} & \resultcell{0.4333}{0.0039504674331652632} & \resultcell{0.2957}{0.0048700580103157648} & \resultcell{0.4278}{0.0022782681105935599} \\
shared, persistent, sync & \resultcell{0.3217}{0.007382642061590867} & \resultcell{0.4487}{0.0042465755436612461} & \resultcell{0.3019}{0.0053053104122193348} & \resultcell{0.4337}{0.0035810874419335737} & \resultcell{0.3068}{0.0047329758262661878} & \resultcell{0.4378}{0.002668313654965265} & \resultcell{0.3019}{0.0053935218231504394} & \resultcell{0.4337}{0.0035955131480475606} \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/encoder_context.tex <==
\begin{table}[t]
\centering
\caption{Two temporal encoders with and without BRIDGE. Five-seed test means under a common forecast loss and checkpoint rule.}
\label{tab:encoder-context}
\begingroup\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.18}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrrr@{}}
\toprule
Model & \multicolumn{2}{c}{HA} & \multicolumn{2}{c}{USHCN} & \multicolumn{2}{c}{P12} & \multicolumn{2}{c}{MIMIC} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
 & MSE $\downarrow$ & MAE $\downarrow$ & MSE $\downarrow$ & MAE $\downarrow$ & MSE $\downarrow$ & MAE $\downarrow$ & MSE $\downarrow$ & MAE $\downarrow$ \\
\midrule
TRCF & \numstat{0.0407}{0.000191143} & \numstat{0.1123}{0.000247643} & \numstat{0.1431}{0.010575315} & \numstat{0.2524}{0.005621037} & \numstat{0.2872}{0.000267297} & \numstat{0.3516}{0.000564862} & \numstat{0.4043}{0.003305092} & \numstat{0.3816}{0.000830660} \\
ANCHOR only & \numstat{0.0409}{0.000181507} & \numstat{0.1127}{0.000209918} & \numstat{0.1365}{0.006842003} & \numstat{0.2498}{0.008043552} & \numstat{0.2884}{0.000633295} & \numstat{0.3517}{0.000582775} & \numstat{0.4222}{0.003215937} & \numstat{0.3919}{0.001240275} \\
Adaptive patches only & \numstat{0.0421}{0.000074189} & \numstat{0.1156}{0.000389054} & \numstat{0.1540}{0.004415841} & \numstat{0.2608}{0.006303324} & \numstat{0.2932}{0.001021718} & \numstat{0.3564}{0.000708939} & \numstat{0.4232}{0.004851228} & \numstat{0.3935}{0.002098423} \\
Adaptive patches + BRIDGE & \numstat{0.0419}{0.000145529} & \numstat{0.1157}{0.000477740} & \numstat{0.1514}{0.010438914} & \numstat{0.2626}{0.009768199} & \numstat{0.2894}{0.000574745} & \numstat{0.3546}{0.001070215} & \numstat{0.4041}{0.001104031} & \numstat{0.3826}{0.000839403} \\
\bottomrule
\end{tabular*}
\endgroup
\end{table}


==> tables/forecast_loss_ablation.tex <==
\begin{table}[H]
\centering
\caption{Forecast-loss ablation. Test means over five paired seeds; only the forecast MAE weight $\alpha$ changes.}
\label{tab:forecast-loss}
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.16}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
Dataset & \multicolumn{2}{c}{MSE} & \multicolumn{2}{c}{MAE} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
 & $\alpha=0$ & $\alpha=0.1$ & $\alpha=0$ & $\alpha=0.1$ \\
\midrule
HumanActivity & \numstat{0.040696}{0.000191} & \numstat{0.040842}{0.000178} & \numstat{0.112347}{0.000248} & \numstat{0.112070}{0.000257} \\
USHCN & \numstat{0.143051}{0.010575} & \numstat{0.138579}{0.009356} & \numstat{0.252372}{0.005621} & \numstat{0.240716}{0.005930} \\
P12 & \numstat{0.287207}{0.000267} & \numstat{0.287606}{0.001745} & \numstat{0.351600}{0.000565} & \numstat{0.350906}{0.002377} \\
MIMIC-III & \numstat{0.404281}{0.003305} & \numstat{0.404830}{0.002145} & \numstat{0.381599}{0.000831} & \numstat{0.380072}{0.001597} \\
\bottomrule
\end{tabular*}
\endgroup
\end{table}


==> tables/inference_memory_compact.tex <==
\begin{table}[H]
\centering
\caption{APN and TRCF: peak inference memory (MiB) and five-seed mean test MSE. The same three validation batches are profiled in FP32 on an RTX 5090. Parameter counts and prediction variability are reported in Appendix~\ref{app:protocol}.}
\label{tab:inference-memory}
\begingroup\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.15}
\begin{tabular}{lrrrrr}
\toprule
Dataset & Batch & \multicolumn{2}{c}{Memory (MiB) $\downarrow$} & \multicolumn{2}{c}{Test MSE $\downarrow$} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
 & & APN & TRCF & APN & TRCF \\
\midrule
HA & 16 & 120.1 & 14.4 & \numstat{0.0421}{0.000105452} & \numstat{0.0407}{0.000191143} \\
USHCN & 32 & 74.1 & 21.1 & \numstat{0.1591}{0.013786464} & \numstat{0.1431}{0.010575315} \\
P12 & 32 & 31.2 & 25.8 & \numstat{0.2947}{0.003096938} & \numstat{0.2872}{0.000267297} \\
MIMIC & 32 & 193.8 & 63.9 & \numstat{0.4323}{0.005553091} & \numstat{0.4043}{0.003305092} \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/partition_robustness.tex <==
\begin{table*}[t]
\centering
\caption{Two additional record partitions with training-history normalization. Three-seed test means per partition.}
\label{tab:partition-robustness}
\begingroup\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.18}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrrr@{}}
\toprule
Model & \multicolumn{4}{c}{USHCN} & \multicolumn{4}{c}{MIMIC} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
 & \multicolumn{2}{c}{Split 31001} & \multicolumn{2}{c}{Split 31002} & \multicolumn{2}{c}{Split 31001} & \multicolumn{2}{c}{Split 31002} \\
 & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
\midrule
Adaptive, original $P$ & \resultcell{0.6201}{0.0074685904914991094} & \resultcell{0.3617}{0.0028690869623553728} & \textbf{\resultcell{0.2408}{0.017916743404520295}} & \textbf{\resultcell{0.2987}{0.0071689105682915585}} & \resultcell{0.4272}{0.0079868845315128421} & \resultcell{0.4007}{0.0047224064548827254} & \resultcell{0.4180}{0.0012721875436191902} & \resultcell{0.3951}{0.0013662892389339578} \\
Adaptive, $P=16$ & \resultcell{0.5995}{0.021814247300813494} & \resultcell{0.3858}{0.021619632284480276} & \resultcell{0.2516}{0.0088841907364223625} & \underline{\resultcell{0.2994}{0.0097036892919884071}} & \resultcell{0.4243}{0.003836558594189853} & \resultcell{0.4002}{0.0021782724497366778} & \resultcell{0.4179}{0.0018804724764543521} & \resultcell{0.3968}{0.0012726746445739484} \\
ANCHOR & \underline{\resultcell{0.5661}{0.035985478605401508}} & \textbf{\resultcell{0.3555}{0.0038796369687106153}} & \resultcell{0.2504}{0.0064986166164329763} & \resultcell{0.3048}{0.01474022871414438} & \resultcell{0.4210}{0.0031684903397723434} & \resultcell{0.3969}{0.0028370393865769991} & \resultcell{0.4161}{0.0010997020060587099} & \resultcell{0.3942}{0.0017962103076032533} \\
TRCF & \resultcell{0.5770}{0.035971703508703615} & \resultcell{0.3635}{0.0027636591324457591} & \resultcell{0.2413}{0.012112498258967829} & \resultcell{0.3023}{0.0088639724685372866} & \underline{\resultcell{0.4058}{0.0023214004403751556}} & \textbf{\resultcell{0.3863}{0.00085769857926011074}} & \underline{\resultcell{0.3999}{0.0016244703472792167}} & \underline{\resultcell{0.3858}{0.00067523716754256541}} \\
Raw relay & \textbf{\resultcell{0.5658}{0.039102827584469618}} & \underline{\resultcell{0.3604}{0.0031974488349689662}} & \resultcell{0.2418}{0.013081405131087435} & \resultcell{0.3038}{0.011135490345590306} & \textbf{\resultcell{0.4036}{0.0032495499099090982}} & \underline{\resultcell{0.3897}{0.0033579649724877411}} & \textbf{\resultcell{0.3971}{0.0031859567414205497}} & \textbf{\resultcell{0.3855}{0.001658845071817433}} \\
Observed residuals & \resultcell{0.5771}{0.03569857970277298} & \resultcell{0.3639}{0.0026273440178915916} & \underline{\resultcell{0.2412}{0.012060060799211618}} & \resultcell{0.3024}{0.0094165058025329883} & \resultcell{0.4122}{0.0042984095673589988} & \resultcell{0.3906}{0.0022699080744399366} & \resultcell{0.4045}{0.001223165687811906} & \resultcell{0.3892}{0.0018326145780300979} \\
\bottomrule
\end{tabular*}
\endgroup
\end{table*}

